QFF: Quantized Fourier Features for Neural Field Representations

Multilayer perceptrons (MLPs) learn high frequencies slowly. Recent approaches encode features in spatial bins to improve speed of learning details, but at the cost of larger model size and loss of continuity. Instead, we propose to encode features in bins of Fourier features that are commonly used for positional encoding. We call these Quantized Fourier Features (QFF). As a naturally multiresolution and periodic representation, our experiments show that using QFF can result in smaller model size, faster training, and better quality outputs for several applications, including Neural Image Representations (NIR), Neural Radiance Field (NeRF) and Signed Distance Function (SDF) modeling. QFF are easy to code, fast to compute, and serve as a simple drop-in addition to many neural field representations.

==> figures/comparison.tex <==
%%%%%%%%% ABSTRACT
\begin{table}[]
    \centering
    \captionsetup{type=figure}
    \begin{tabular}{c}
        \includegraphics[width=0.8\textwidth,keepaspectratio]{figures/PE.pdf}\\
        \includegraphics[width=0.8\textwidth,keepaspectratio]{figures/voxel.pdf}\\
        \includegraphics[width=0.8\textwidth,keepaspectratio]{figures/triplane.pdf}\\
        \includegraphics[width=0.8\textwidth,keepaspectratio]{figures/QFF.pdf}
    \end{tabular}
\captionof{figure}{Comparison between }
\label{fig:representation}
\end{table}

% \includegraphics[width=0.6\textwidth,keepaspectratio]{images/qff_teaser.png}
\label{fig:overview}
% \end{figure*}

==> figures/mega_pixel.tex <==
\begin{figure}
    \centering
    \begin{tabular}{cc}
        \tikz{ 
        \node[draw=black, line width=.4mm, inner sep=0pt](gt) at (0,0){\includegraphics[trim={0 0 0 6cm},clip,width=0.23\textwidth]{images/mega_pixel/gt_2.png}};
        }& 
        \tikz{ 
        \node[draw=black, line width=.4mm, inner sep=0pt](gt) at (0,0){\includegraphics[trim={0 0 0 6cm},clip,width=0.23\textwidth]{images/mega_pixel/base_2.png}}}\\
        Ground Truth & ReLU \\
        \tikz{ 
        \node[draw=black, line width=.4mm, inner sep=0pt](gt) at (0,0){\includegraphics[trim={0 0 0 6cm},clip,width=0.23\textwidth]{images/mega_pixel/pe_relu_2.png}}} & 
        \tikz{ 
        \node[draw=black, line width=.4mm, inner sep=0pt](gt) at (0,0){\includegraphics[trim={0 0 0 6cm},clip,width=0.23\textwidth]{images/mega_pixel/freq_cp_relu_2.png}}}\\
        Pos. Enc. ReLU & \textit{QFF-Lite} ReLU
    \end{tabular}
    \caption{
        \textbf{Comparison of supervised image reconstructions.} ReLU refers to MLP without any encoding. Pos. Enc. ReLU refers to ReLU network with Positional Encoding, and \textit{QFF-Lite} ReLU refers to ReLU network with \textit{QFF-Lite} encodings.
    }
    \label{fig:megapixel}
\end{figure}
% \end{figure*}

==> figures/temp.tex <==
    {\tikz{
    \node[draw=black, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (0, 0) {\includegraphics[width=0.19\textwidth]{images/scannet/scan_1_gt_piano.png}};
    \node[draw=green, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (-.9, -.9) {\includegraphics[trim=6cm 14cm 18cm 10cm, clip, width=0.08\textwidth]{images/scannet/scan_1_gt_piano.png}};
    }} & 
    {\tikz{
    \node[draw=black, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (0, 0) {\includegraphics[width=0.19\textwidth]{images/scannet/scan_1_mlp_piano.png}};
    \node[draw=green, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (-.9, -.9) {\includegraphics[trim=6cm 14cm 18cm 10cm, clip, width=0.08\textwidth]{images/scannet/scan_1_mlp_piano.png}};
    }} & 
    {\tikz{
    \node[draw=black, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (0, 0) {\includegraphics[width=0.19\textwidth]{images/scannet/scan_1_grid_piano.png}};
    \node[draw=green, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (-.9, -.9) {\includegraphics[trim=6cm 14cm 18cm 10cm, clip, width=0.08\textwidth]{images/scannet/scan_1_grid_piano.png}};
    }} & 
    {\tikz{
    \node[draw=black, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (0, 0) {\includegraphics[width=0.19\textwidth]{images/scannet/scan_1_qff_lite_piano.png}};
    \node[draw=green, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (-.9, -.9) {\includegraphics[trim=6cm 14cm 18cm 10cm, clip, width=0.08\textwidth]{images/scannet/scan_1_qff_lite_piano.png}};
    }} & 
    {\tikz{
    \node[draw=black, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (0, 0) {\includegraphics[width=0.19\textwidth]{images/scannet/scan_1_qff_3d_piano.png}};
    \node[draw=green, draw opacity=1.0, line width=.3mm, inner sep=0pt](qff) at (-.9, -.9) {\includegraphics[trim=6cm 14cm 18cm 10cm, clip, width=0.08\textwidth]{images/scannet/scan_1_qff_3d_piano.png}};
    }} \\


==> tables/ablation_noadd.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l| c c | c}
\toprule
Method                              & Adding Pos. Enc.  & PSNR \\
\midrule
\multirow{2}{*}{\textit{QFF-Lite}} 
& $\times$      & \\
& $\checkmark$      & \\
\midrule
\multirow{2}{*}{\textit{QFF-3D}}
& $\times$      & \\
& $\checkmark$      & \\
\bottomrule
\end{tabular}

\caption{
    \textbf{Evaluation on supervised Neural Image Representation.} The best performing method per dataset for each activation functions are marked as bold. 
}
\label{tab:megapixel}
\end{table}

